AutoSynth: Learning to Generate 3D Training Data for Object Point Cloud Registration

In the current deep learning paradigm, the amount and quality of training data are as critical as the network architecture and its training details. However, collecting, processing, and annotating real data at scale is difficult, expensive, and time-consuming, particularly for tasks such as 3D object registration. While synthetic datasets can be created, they require expertise to design and include a limited number of categories. In this paper, we introduce a new approach called AutoSynth, which automatically generates 3D training data for point cloud registration. Specifically, AutoSynth automatically curates an optimal dataset by exploring a search space encompassing millions of potential datasets with diverse 3D shapes at a low cost.To achieve this, we generate synthetic 3D datasets by assembling shape primitives, and develop a meta-learning strategy to search for the best training data for 3D registration on real point clouds. For this search to remain tractable, we replace the point cloud registration network with a much smaller surrogate network, leading to a $4056.43$ times speedup. We demonstrate the generality of our approach by implementing it with two different point cloud registration networks, BPNet and IDAM. Our results on TUD-L, LINEMOD and Occluded-LINEMOD evidence that a neural network trained on our searched dataset yields consistently better performance than the same one trained on the widely used ModelNet40 dataset.

==> fig/arch_comprison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{image/arch_comprison.pdf}
    \caption{Comparison of the different architecture. S is short for simulator. Note that our method could also merge with the existing reinforcement learning and evolutionary based surrogate model pipeline.}
    \label{fig:arch_comp}
\end{figure}

==> fig/embedding_dims.tex <==
\begin{*figure}
    \centering
    \includegraphics{image/emb_curve.png}
    \caption{Caption}
    \label{fig:emb_dims}
\end{*figure}

==> fig/latent_space.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/bunny_perplexity45_nsample_100.png}
    \includegraphics[width=\linewidth]{image/modelnet_perplexity45_nsample_300.png}
    \caption{T-SNE visualization of the latent space feature produced by the encoder. }
    \label{fig:latent_space}
\end{figure}

==> fig/mesh_vis.tex <==
% \begin{figure}
%     \setlength{\belowcaptionskip}{-1.em}
%     \centering
%     \includegraphics[width=.085\textwidth]{image/primitive_vis/cone.png}
%     \includegraphics[width=.085\textwidth]{image/primitive_vis/cuboid.png}
%     \includegraphics[width=.085\textwidth]{image/primitive_vis/cylinder.png}
%     \includegraphics[width=.085\textwidth]{image/primitive_vis/dodecahedron.png}
%     \includegraphics[width=.085\textwidth]{image/primitive_vis/octahedron.png}
%     \includegraphics[width=.095\textwidth]{image/primitive_vis/icosahedron.png}
%     \includegraphics[width=.095\textwidth]{image/primitive_vis/sphere.png}
%     \includegraphics[width=.095\textwidth]{image/primitive_vis/torus.png}
%     \includegraphics[width=.095\textwidth]{image/primitive_vis/tetrahedron.png}
%     \includegraphics[width=.085\textwidth]{image/mesh_sa/1.png}
%     \includegraphics[width=.085\textwidth]{image/mesh_sa/2.png}
%     \includegraphics[width=.085\textwidth]{image/mesh_sa/3.png}
%     \includegraphics[width=.085\textwidth]{image/mesh_sa/4.png}
%     \includegraphics[width=.085\textwidth]{image/mesh_sa/5.png}
%     \caption{Primitives (blue) and AutoSynth shapes (yellow).\ZD{We can replace this with the one that illustrate the process and result that applying each operation to the shape primitives.}}
%     \label{fig:mesh_vis}
% \end{figure}

\begin{figure*}[ht]
    \setlength{\belowcaptionskip}{-1.em}
    \centering
    \includegraphics[width=0.9\linewidth]{image/search_space.png}
    \caption{Primitives (blue) and AutoSynth shapes (yellow).\ZD{Need to emphsis the evolution procedure.}}
    \label{fig:mesh_vis}
\end{figure*}

==> fig/overview.tex <==
\begin{figure}
    \setlength{\belowcaptionskip}{-1.em} 
    \centering
    \includegraphics[width=\linewidth]{image/flow_fig.pdf}
    \caption{Overview of the search phase.}
    \label{fig:overview}
    \setlength{\belowcaptionskip}{-15pt}
\end{figure}

==> fig/rebuttal_bunny_angle.tex <==
% \begin{figure}
%     % \setlength{\belowcaptionskip}{-1.em} 
%     \centering
%     \includegraphics[width=.5\linewidth]{image/bunny_angle.png}
%     \caption{Artifacts in the Stanford Bunny angle.}
%     \label{fig:rebuttal_bunny_angle}
%     % \setlength{\belowcaptionskip}{-15pt}
% \end{figure}

\begin{wrapfigure}{r}{0.2\textwidth}
  \begin{center}
    \includegraphics[width=\linewidth]{image/bunny_angle.png}
  \end{center}
  \caption{Artifacts in the Stanford Bunny angle.}
\label{fig:rebuttal_bunny_angle}
\end{wrapfigure}

==> rebuttal_tex_cvpr/R1.tex <==
 %\section{To R1}

\noindent{\bf To PDAW}

\noindent{\bf Q1: Choice of primitives.} The choice of primitives and transformations is technically unrestricted. In this work, we adopt a pragmatic approach and choose shape primitives and transformations that are simple enough to maintain the cost of generating a dataset low while allowing us to obtain complicated and diverse objects by combining them. We do not claim these choices to be optimal. However, our meta-learning approach explicitly searches for the best combinations in this space, and our experiments evidence these choices to be sufficient to yield SOTA results. Fig.~1 only illustrates a few cases, and we will include more.

%Increasing the variety of those two may lead to a new SOTA than what we presented.  The method demonstrates to be a quick, inexpensive strategy to enhance the performance of geometric-related tasks by introducing more shape varieties. And only a small percentage of the objects we generated are shown in Figure 1, and the final version will feature more diversified geometry.

% We here takes a practical way that links the data synthesis process with the data evaluation process, hence the latter would direct the former and in the end generate appropriate synthetic dataset for the targeted task network. In such a meta-learning fashion, the approach allows us to quickly produce synthetic datasets that aim to improve the performance of the target task network. It is worth to mention that each best policy searched indeed determines an upper bound for the weighting of each transformation, and numerous objects can be generated from this range. Practically, we randomly sampled objects from the range in each iteration for all batches, which yields 50000*32 objects. Figure 1 simply displays some objects of the synthetic datasets that exhibit as intersections of simple shapes. On one side, this simple transformation will also produce new facets, new angles, and new polygons. On the other hand, our generated datasets indeed have more other complex objects produced from shear, stretch, etc. 

% reconstrcution -> chamfer distance, 形状见过的越多则越容易重建出未见过的物体->chamfer distance会减小；
% registration ->训练中见到的diversity越多，那么unseen的时候没见过的就越少，越容易进行泛化-> registration 的结果就会越好。

\noindent{\bf Q2: Surrogate model.} 
Our choice of surrogate model was motivated by (i) its computational cost and (ii) its similar behavior to the registration one in the presence of varying number and diversity of the training data. The former rules out any registration network because we observed that reducing registration architectures sufficiently made them produce meaningless results. We therefore turned to a reconstruction network, which does not require additional annotations, and, as shown in Table 4 in the paper and Table 2 in the sup. mat., exhibits a trend consistent with registration performance when tested on TUD-L, LM, and LMO.

%The number of shape varieties in the training process similarly affects the generalization and the performance of registration and reconstruction networks. Table 4 in the paper and Table 2 in the supplementary exhibit a consistent tendency between the registration performance and the reconstruction error when tested with TUD-L, LM, and LMO datasets. Though offsets exist between these two networks, their similarity is also justifiable.

% More shape features are supposed to improve the generalization of both networks (i.e., more shape features 'seen' in the training results in less shape features 'unseen' in the testing) and lead to increased registration performance and reduced reconstruction error, as evidenced by Table 4.
% Furthermore, Table 2 in supplementary displays the same dependency between the registration performance and reconstruction error when tested on LM and LMO. 
% Though offsets exist between these two types of networks, this is the optimal choice we have. The BPNet we applied in this paper is in fact among the smallest registration networks and contains simply 6MB of learning parameters, it requires a minimum of $30,000$ GPU hours on an RTX8000 for policy searching from our estimation. 

% The shape sensitivity of both the reconstruction and registration network enables the former to server as a surrogate model for the latter. 
% Increasing diversity of shape in training data improves the reconstruction by reducing the chance of encountering unseen geometric features during testing. 
% The same applies to registration, where increasing diversity of shapes in training data reduces the occurrence of unseen geometry structures, leading to better generalization and improved registration performance. 
% Our experiments support this, as shown in Tab. 4 where increasing shape diversity in the training dataset raises registration performance and reduces Chamfer distance error in the reconstruction task. 

% Contrary to the belief that a smaller registration network can serve as a surrogate model, the answer is no. BPNet, the smallest one-shot registration model known to us, still contains 6MB of learning parameters and requires a minimum of $30,000$ GPU hours on an RTX8000 for searching.
% Point cloud tasks like segmentation, detection, and classification require data annotation and focus on semantic shape meaning, not shape variety. Detection also adds additional computational effort to rendering the background. 

% While reconstruction was chosen as the surrogate model due to its shape sensitivity, popular models like NeuralPoints, PU-GAN, and PU-Net have too many parameters and take shortcuts,resulting in a copy and paste of the input point set. Improving and shrinking these networks is not a trivial task. Our solution was to design a small autoencoder that performs effectively.


\begin{comment}
Firstly, the BPNet we have chosen is the smallest one-shot registration model up to our knowledge which contains simply 6MB of learning parameters; however it requires at least $30,000$ GPU hours on an RTX8000 to finish the training process when it was set as a target task network in the automatic machine learning framework. Alternatively, we replaced the registration network with a surrogate network to make the framework approachable. The surrogate network should have a similar dependency with object shapes as the registration network has, but is way much faster to run. Theoretically, point cloud segmentation, detection, classification, and reconstruction would serve as candidates for the surrogate network. However, the point cloud segmentation and classification task require data annotation and focuses on the semantic meaning of shapes rather than the shape varieties that we value; the point cloud detection task would introduce further computational effort to add a scene point cloud. We believe the reconstruction task works properly here because the shape variety matters. Among a variety of reconstruction models,including NeuralPoints, PU-GAN, and PU-Net, they still possess too many parameters and often take a shortcut, resulting in a copy and paste of the input point set. Improving and shrinking these networks is not a trivial task. Instead, we designed a small autoencoder that effectively performs the task. It is observed that synthetic training data do have a similar effect on the performance of both tasks: the increasing of the registration performance accompanying the decreasing of the reconstruction error.

% Q2: The surrogate model must meets two requirements: 1) Must be sensitive to the shape. 2) Must be extremely fast in the training process. The model which takes the point cloud as input are, registration, segmentation, reconstruction, detection, tacking. These task model can be considered as shape sensitive model. However, the primitive shapes doesn't contains the semantic meaningful parts, thus the segmentation is excluded. Since we only care about the object itself, thus the detection and tracking is excluded. The rest two possible task is recontruction and registration. The BPNet is one of the smallest registration model which only contains 6MB learning parameters, but train it requires 30 GPU hours on an RTX8000. The reconstruction model we have tried the XXX, XXX and XXX, however, these models possesses too many parameters, thus they always find a short cut which acts like copy and paste the input point set. Thus, we decide to design a small network, which first encode the original point set to the latent feature, and then decode the shape from the latent feature.
\end{comment}


\noindent{\bf Q3: Ranking shapes based on uncertainty.} This is an interesting idea. However, this would require designing an uncertainty measure for our task, which differs from the typical recognition scenarios used in active learning. We are not aware of any effort going in this direction but will keep it in mind for future work.

%Optimizing a single shape through active learning is simpler than generating multiple datasets and ranking them, but it also greatly increases the risk of network overfitting. We've made similar attempts but failed due to overfitting.
% attempted to generate complex shapes for the registration task. The experiment quickly reach the highest performance within $1,000$ iterations during training, but achieves poor performance on the testing dataset.
\begin{comment}

Suppose that we successfully generate a group of diverse shapes and use the same sampling strategy in the registration task as what we do with selected diverse datasets (i.e., uniformly sampling $1,024$ points from the surface of each object's mesh model), the data
If we use the same method sampling points from the surface of shapes. The 
In the registration task, if we apply the same sampling strategy to the selected shapes and the selected datasets 
uniformly sampling $1,024$ points from the surface of the object's mesh model in the training process. 
To overcome this problem, we generate new shapes in each batch iteration using the policy-defined value range. Over the entire training process, we generate up to $50000\times 32$ unique shapes, exposing the network to $1.6384\times 10^9$ unique structures, reducing the risk of overfitting.
The DGCNN feature extraction module builds a graph structure for each point, which includes the point and its 20 neighboring points. Despite augmenting the input coordinates through rotation or different surface sampling methods, the graph structure remains similar, leading to overfitting of the 1,024 structures and deteriorated performance on the unseen test dataset.


to the fixed number of points $1,024$ sampled from the shape's surface. 
The network's tendency to take shortcuts makes it easier to overfit the points' coordinates of single object than to learn a concise, expressive shape descriptor which able to generalize to unseen object. 
Spreading the variety across multiple shapes, through random arrangements and combinations of unique features, results in a large number of diverse shapes, making it impossible for the network to overfit all the coordinates, instead, it develops the ability to find valid descriptors.


% Combining all complex 3D features to form a single object is a difficult task as the most challenging part is no clear criterion for determining useful features. 
The main challenge in high-level structuring a single shape is to find a concise and expressive abstract description of shapes that can be useful for improving the target task performance. 
This challenge also arises when designing a shape set. To overcome this, we use meta-learning with a feedback loop. We extract evaluation performance feedback from the target task network trained on the generated dataset, and use it to guide the design of the shape set.
% To the best of our knowledge, we are the first to apply meta-learning to the point cloud registration task.

The central idea of active learning is to put weights on each shapes, similarly, our meta-learning framework can also be considered as putting weights on each shapes through putting weights on the policy parameters. Active learning aims to create a dataset that performs well on the random shapes, but this doesn't guarantee an improvement on the target dataset. In contrast, our meta-learning method explicitly incorporate the performance of the target dataset in the feedback loop, making it more directional and effective than active learning.

% The network samples a fixed number of points, specifically $1,024$, from the surface of an object. However, if an object has a high number of unique 3D features, the number of points allocated to represent each feature decreases, which can impede effective learning. Increasing the number of sampling points will result in a quadratic increase in computational and memory costs. Additionally, if the object is significantly different from those in the testing dataset, it may result in poor generalization ability of the network model.

% 1. 他这里是在说从生成的数据里面选择吗？应该不是从modelnet40数据里面进行选择吧。
% 2. 他这里需要一个初始的网络吧，这个初始的网络该如何进行选择呢？
% 3. 他这里面也需要不断的iteration，

% Design a single object which contains the all the unique feature is a challenging task, as it's difficult to measure the different
% We using numerous shapes instead of single complex shape is to avoid the overfitting. Emperically speaking, the network need to be large enough to able to generalize to the unseen object. However, the larger the network is, the easier for the network to overfit the training object. The use of different shaped objects as training data can effectively prevent the network from overfitting to a particular shape.
\end{comment}

\noindent{\bf Q4: Shape constraints.} Thank you for pointing this out. We indeed impose constraints on the size of the primitives, and the magnitude of translation, scaling, and other transformations
%, such as [0.1,1] for scaling and [-1,1] for translation range. 
We have observed this to drastically reduce the presence of floating primitives. We will clarify this.
%Floating situations are uncommon, according to random samplings we've done on the created objects. Additionally, the floating cases and intersecting cases are evaluated using the same criteria: the most diverse ones are maintained, while the rest are excluded.

% We establish constraints on the minimum enclosing cube, translation and scaling of shape primitives to ensure their intersection with each axis is in the range of -1 to 1, and translation is between -1 to 1, and scaling between 0.1 to 1. 

% These constraints reduce the chances of separation among the primitives. Before union operation, we impose transformations and mesh truncation to the shapes. This makes it unlikely for any floating objects to match the original shape exactly. During the search phase, we use meta-learning to select the policy that is relevant to a diverse dataset. The policy without sufficient shape diversity will be eliminated.


\begin{comment}
We set the minimum enclosing cube of all the shape primitives intersecting with each axis in the range of -1 to 1, and the translation ranging from -1 to 1, and the scaling ranging from 0.1 to 1. With these constraints, we reduce the possibility of separating from each other. Since we impose the transformations and mesh object truncation operation to the primitive shapes before union operation. So even if a floating object appears in our set-up it is unlikely to be exactly the same as the original shape. In the searching phase, we use meta-learning to select the policy which related to the dataset with abundant shape diversity. The one without will be phased outed.

Constraints
has the possibility of generating floating shapes, but not singulated primitives, as XX is enforced
the shapes consits of floating transformed primitives (if not contain abundant local features, will be taotai by the plicy search process,


At first, we indeed set some constraints to the scale, translation and primitive shape size. To be specific, the minimum enclosing cube of the shape primitives is restricted to the interval $[-1,1]$ on each axises. 

We limited the translation which is added to each primitives within the range $[-1, 1]$, 

and the scale which is multipled to each primitives before merging within the range $[0.1, 1]$. 

Thus there is a small amount of separation of objects in our case. Since we impose the transformations and mesh object truncation operation to the primitive shapes before union operation. So even if a floating object appears in our set-up it is impossible to be exactly the same as the original shape. We will clarify this in the final version.
\end{comment}



% 1. 这两个数据集都属于secene level， scene level 数据用在object level会有什么样的问题。除了model net40外，还有shapenet，我们也得到了较好的比较结果。
% 2. object level realistic数据集有哪些，数量都非常的少。
\noindent{\bf Q5: Other datasets.} ICL-NUIM and SUN3D are scene-level datasets. We focus on object-level point cloud registration, which motivated our way of generating training data. In this context, ModelNet40 is the most widely used dataset, but we nonetheless also report results on the real TUD-L, LM, and LMO datasets in Tables 1--3.

% These two datasets are both the scene-level point cloud datasets, however, our paper only focus on the object-level point cloud registration which we will clarify in the final version.

% To extract point cloud of objects from these datasets is a tremendous undertaking. There is also a lack of real-scene datasets to match the number of objects in the ModelNet40. For the real scene object training result, we provide the result on the TUD-L, LM and LMO dataset. BPNet-real is trained on the real-scene training data provided by the dataset, which has the same objects as the testing dataset. Although the BPNet trained on our AutoSynth generated dataset has not seen any object from the testing dataset, it still managed to get a good result. Using our AutoSynth generated dataset as the pre-training model and then fine-tune on the TUD-L dataset can achieves better performance than the one trained from scartch on the TUD-L, as shown in the Table~\ref{tab:rebuttal_tudl}.

% In table XXX, we also provide the result which trained on the TUD-L real-scene dataset. This dataset can be consider as the upper bound performance of the algorithm. The key to the generalization ability to the network is the diversity of the dataset. Even the object contains in the SUN3D and ICL-NUIM is more realistic, but due to the limited shape diversity, it will also induces the limited performance. More importantly, the capturing and annotation process of SUN3D and ICL-NUIM dataset require large amount of human laber work. In contrast, we only needs 1$\sim$ 2 GPU days.



==> rebuttal_tex_cvpr/R2.tex <==
\noindent{\bf To Zxdy}


% 1. meta-learning zenme work
% 2. 用你妈都没事儿，11个shape并不多，而ModelNet40的shape是远远的多余我选择的shape的。
% 3. meta-learning 自己选择的，从我们的经验来说，shearing， scale，strestch，union的影响很大
% 4. registration做不来哦
% 5. 50000*32
\noindent{\bf Q1: Synthetic data quality.} 
Please see PDAW-Q1. Ultimately, we define a shape space that is computationally tractable while letting us generate complicated shapes. Our meta-learning approach then searches for the best combinations in this space. Unfortunately, using a smaller registration network is not an option; BPNet is one of the smallest registration networks, with 6MB of parameters, and it would require at least $30,000$ GPU hours on an RTX8000 for policy searching. We have observed that reducing it to the point where it becomes practical makes it produce meaningless results.
We acknowledge that our choices may not be optimal, but our experiments evidence that they are sufficient to yield SOTA results. We will clarify this.

%We believe the quality of generated datasets originated from the arrangments and combinations of shapes and chose 11 shape primitives to testify this hypothesis. Practically, we combine data synthesis with data evaluation, with the latter guiding the former in selecting suitable datasets for the targeted task network. The numbers and the geometry characteristics of chosen shape basis, as well as the designed transformations, define the search space and affect the task performance. Systematic investigations on these variables are worthwhile to realize the full potential of synthetic datasets. In this study, we found that 11 primitive-shape-based objects ($50000\times 32$ shapes) outperform ModelNet40, which contains $12, 311$ objects; and transformations such as scaling, rotation, shearing, stretching, and union are more significant than others. BPNet we used is one of the smallest registration networks with 6MB of learning parameters. Based on our estimation, it requires a minimum of $30,000$ GPU hours on an RTX8000 for policy searching. Instead, we used a surrogate model, and the justification is provided in PDAW-Q2.

% The meta-learning mechanism plays a vital role in enhancing the performance of primitive shapes. It achieves this by taking feedback from network training and using it to direct the creation of complex shapes. 11 primitive shapes are already three orders of magnitude smaller than the ModelNet40 which contains $12, 311$. The meta-learning algorithm determines the most critical transformations through feedback from network training and evaluation. Scaling, rotation, shearing, stretching, and union operations were found to be significant through empirical study. The BPNet used in this paper is one of the smallest registration networks with 6MB of learning parameters. It requires a minimum of $30,000$ GPU hours on an RTX8000 for policy searching, based on our estimation. In practice, we use $50000\times 32$ shapes for training.

% We here takes a practical way that links the data synthesis process with the data evaluation process, hence the latter would direct the former and in the end generate appropriate synthetic dataset for the targeted task network. In such a meta-learning fashion, the approach allows us to quickly produce synthetic datasets that aim to improve the performance of the target task network. 

\input{rebuttal_tex/mix_model.tex}
\noindent{\bf Q2: Mixing synthetic and real data.} Finding a good ratio to directly mix synthetic and real data is difficult, particularly since only limited numbers of real samples are available. Instead, to nonetheless follow the reviewer's suggestion, we pre-trained the network on the AutoSynth-searched data and fine-tuned it on the TUD-L training set. This let us reach a new SOTA performance (\textbf{0.94} in R$5^{\circ}$ mAP, see Tab.~\ref{tab:rebuttal_tudl}), showing the effectiveness of our AutoSynth dataset. Thank you for this suggestion, we will include these results.
%in improving existing methods through better initial network parameters.
% 1. bunny bingbu jian dan,真实数据就是没有完美的点线面；
% 2. refer to surrogate合理性

\noindent{\bf Q3: Surrogate model.} Please see PDAW-Q2. Note that the Stanford bunny is not as simple and smooth as it may seem. Moreover, an important gap between synthetic and real objects is that the geometric features of the former are perfect while that of the latter are not. Therefore, our meta-learning strategy favors policies that better match such imperfect geometric features. Our comparisons of AutoSynth vs ModelNet40 training validate the effectiveness of this approach.

%When using a bunny as the target dataset for evaluating the synthetic datasets, the policies favour those that contain similar geometry features as the bunny. The results of bunny and ModelNet40 validate our approach to bridging the gap.

% complex data with non-smooth surfaces, making it challenging to model real-scene data with imperfect points, lines, and planes. The gap between real and synthetic data is reduced by our meta-learning, which uses feedback from bunny to improve the dataset design. The results on real data further validate our approach in bridging the gap between real and synthetic data.
% For the reason behind using the surrogate model, refer to R1-Q2 for detailed explanation.

==> rebuttal_tex_cvpr/R3.tex <==
\noindent{\bf To 9niM}

\noindent{\bf Q1: Evolutionary search.} We use the algorithm from [46]. In each competition, it retains the best policy found and, based on it, creates a mutation distinct from the existing policies. Thus the policy pool does not shrink. Specifically, the best policy is mutated by randomly altering one of its attributes (i.e., transformation parameters in our case). While we do not use cross-over, we agree that it is worth trying as it might yield more diverse populations. We will discuss the evolutionary search in more detail in the final version.

%The value of each attribute acts as a label in the searching phase and serves as an upper bound in training. The strategy allows us to find a relatively good solution quickly. The cross-over is worth trying as it produces more diverse populations; while it could take longer to run, it yields superior outcomes.
% The search space of policy was defined by 11 discrete value vectors of operations, and the picked policy as well as its mutations are all stored as categorical vectors. For example, the rotation can be divided into 9 parts with $\frac{\pi}{8}$ as interval, each part simultanouelsy corresponds to a distinct label, and mutation occurs by labelling change on the rotation attribute. During training, the value encoded in each catergorical vector will act as the upper bound value with zero as the lower bound. 

%For example, we divid the rotation by $\frac{\pi}{8}$ to get nine values and make them corresponding to different labels. During the training, these labels will be set to the upper bound of the value range, e.g. $\frac{3\pi}{8}$ -> [0,\frac{3\pi}{8}$.

% Unlike conventional genetic algorithms where both parents are kept and mutated through cross-over and mutation, we only retain the best one and delete the worst in each competition. 
% To maintain population size, new offspring are generated by mutating a copy of the best individual. (first copy, the pool size wont shrink, then mutate, what kind of mutate, categorical? details)
% Mutation randomly changes one parameter in the best policy, but with the guarantee that there will be no duplication of any of the previous results, which 
% consists of 11 values each corresponding to a specific discrete label (e.g. rotation is divided by $\frac{\pi}{8}$ with each $\frac{\pi}{8}$ interval increase corresponding to a label). We will clarify this part in the final version.

% This allows us to quickly find a relatively good solution in the population and optimize in its vicinity, resulting in fast convergence to a local optimum.  
% Our algorithm also can switch to use cross-over for evolving new diversed populations, which may take longer to converge, but can reach closer to the global minimum. 
% (Use the cross over strategy may lead to better solution and worth to try, but rquires longer time)

% About the mutation, we randomly change one parameter from the copy of the best policy which consist of 11 values, each value in the policy corresponding to a specific discrete label. For example, for the rotation, we divide it by $\frac{\pi}{8}$, with each $\frac{\pi}{8}$ increase in the interval range corresponding to a specific discrete label.

%A policy can only remain in the population if it is constantly winning the competition. In the end, we will pick the one with highest performance score to be the final policy.
\noindent{\bf Q2: Metropolis-Hastings sampling.} Thank you for the suggestion. While the search algorithm is not our contribution, we agree that this direction is worth exploring.
%We appreciate the suggestion of formulating it as a proper Metropolis-Hastings sampling when a good proposal distribution is found. It is absolutely worth exploring to optimize the efficiency of the algorithm. 

\noindent{\bf Q3: Transformation parameterization.} $\alpha$ encodes a subset of the $T_{stretch}$ operation (global vs axis-wise scaling). We keep it because we expect this to facilitate the use of global scaling during the search.
%we still chose to keep it as it allows us to monitor the contribution of every single object when merging to form a complex object for potential in-depth shape analysis.

% Thank you for bringing this up. Both $\alpha$ and $T_{stretch}$ serve distinct purposes in our transformation parametrization (4). 
% Thank you for bringing up the similarity of our evolutionary algorithm to MCMC sampling. While it is true that our algorithm is heuristic, we have found it to be effective in finding good solutions in our task. However, we acknowledge that formulating it as a proper Metropolis–Hastings sampling would lead to improvements in efficiency if a good proposal distribution can be found. We will consider exploring this possibility in future work.

% We agree that $T_{stretch}$ can concurrently perform the duties of $\alpha$. We keep the $\alpha$ is for the conveniently checking the overall size of the each single object when merging to the complex object. We believe it can be omited for the sake of formal simplicity and the reduction of parameters.
% Thank you for bringing this up. Both $\alpha$ and $T_{stretch}$ serve distinct purposes in our transformation parametrization (4). 
% 1. reason to combine
% 2. reason to separate
% While $T_{stretch}$ can perform the duties of $\alpha$, $\alpha$ provides an additional level of granularity in assessing the size of individual objects during merging into a complex object. We believe this extra level of control allows for greater flexibility in the model and optimizes its performance. However, if deemed necessary, we are open to exploring the possibility of reducing the number of parameters by omitting $\alpha$ in future work.

% Q3: Thank you for your constructive comments. 
%The BPNet we applied in this paper is in fact among the smallest registration networks and contains simply 6MB of learning parameters, it requires a minimum of $30,000$ GPU hours on an RTX8000 for policy searching from our estimation. 
\noindent{\bf Q4: Registration loss.} We agree that using a registration loss would be better than a proxy one. However, as discussed in PDAW-Q2 and Zxdy-Q1, we had to rule out this option because it offers no good  speed/accuracy trade-off.
%registration networks are either too costly or not effective enough.
%It is true that monitoring a registration loss is better than a proxy loss, we clarified our motivation in Zxdy-Q1.


==> rebuttal_tex_iccv/R1.tex <==
\noindent\textbf{To R1}

\noindent \textbf{Comparison with FMR.}
We acknowledge that FMR is a SOTA method for 3D object-based registration. Our experiments with FMR, as summarized in Table~\ref{tab:r1}, resulted in an inferior performance. We attribute this discrepancy to different sampling strategies. Our approach involves sampling the source point set from the surface of object's mesh model, and the target point set from a single camera view of partial object's surface, similar to how a depth camera captures objects. This sampling method can introduce featureless surfaces, requiring a network capable of handling ambiguity. In contrast, FMR samples points from mesh's vertices set, resulting in numerous unique features that are suitable for calculating the feature-metric projection error between point clouds. In practice, adding an ambiguity-handling module could potentially improve FMR's performance. We appreciate your insight in pointing out this paper, and we will explore this subject in future work.

% In our view, the performance of FMR could potentially be boosted by integrating a graph structure, which would further augment the uniqueness of these features. 

% - FMR, SOTA, end-to-end learning-based method
% - FMR, sampling from the mesh’s vertices, result in a lot of unique features, suitable for calculating the feature-metric projection error of two point clouds.
% - BPNet, sampling sampling source points set from the surface of the object’s mesh model, and target point set from the single camera view of partial object’s surface, (similar to the how depth camera samples objects), results in a lot of featureless surfaces, requires the network capable of processing ambuiguity.
% - FMR result originated from sampling 方式, 加graph, 增强feature uniqueness, 让FMR 在这个pipline下面工作

% Thank you for your feedback. 
% While FMR [1] is indeed an effective method, it is designed to tackle a different aspect of the task from what our method addresses. 
% Specifically, FMR excels at \emph{scene-level} registration, which typically benefits from rich features.
% By contrast, our method targets \emph{object-level} registration, which usually deals with 
% %smoother, less feature-dense areas
% sparser and poorer features. Our methodology aligns with BPNet [1], sampling points from the surface of the objects' mesh, which is more akin to real-world scenarios. 
% These differences in focus and methodology translate to an inferior performance of FMR on object-level registration, as shown in Table~\ref{tab:r1}. We will clarify this point in the final version.

\input{table/rebuttal_R1}

\noindent \textbf{Partially-overlapping point clouds.} 
Our study uses a partial-overlap scenario, with the source point set encompasses the entire object and the target set depicts a partial observation from a single-camera view. We'll clarify to avoid confusion.
% The setup in our study indeed is a partial-overlap scenario, where the source point set encompasses the entire object while the target point set depicts a partial observation of the same object, captured from a single-camera viewpoint. We will clarify this to prevent any misunderstanding.

% The setting we use in the article is indeed partial-overlap. As the source point set represents the whole object, and the target point set represents the partial observation of the full object from a single camera view. We will clarify this in our final version.


% We primarily address the partial-overlap scenario in which the target point cloud is acquired from a depth map of a single camera view. This method results in a partial observation of the full object. We will clarify this aspect in our final version.



==> rebuttal_tex_iccv/R2.tex <==

\noindent \textbf{To R2}

% \input{fig/rebuttal_bunny_angle}
\noindent \textbf{Scan data as target dataset.} 
We agree with the reviewer's comment regarding the preference for using real scans over augmented rotations. However, the multi-view partial scans data from the Stanford bunny repository poses a limitation due to artefacts from occlusion-induced false connections, resulting in sub-optimal algorithm performance. This issue is evident in Table 2, specifically the AS-Angle row, where these scans were used as the target dataset. To overcome this, we opted to augment the dataset alternatively.

% We agree with that is more appropriate to use real scans of the same object than using a single object with augmented rotations. However, the Stanford bunny repository's multi-view partial scans present a specific challenge. These scans contain unrealistic connections between unrelated vertices, resulting in suboptimal algorithm performance. This can be observed in Table~\ref{tab:r2} under the AS-Angle row, where these scans from various Stanford bunny perspectives were used as the target dataset.

\noindent \textbf{Applicability to different target datasets.}
We appreciate the reviewer's insight and suggestions regarding the impact of the target dataset choice on our method's performance. We've tested various objects, such as the Stanford bunny and dragon, and results in Table~\ref{tab:r2} confirm our method's consistent SOTA performance. We will incorporate additional real-world objects in the revised Table 5 to thoroughly evaluate our approach.
% Following the reviewer's advice, we'll add more real-world objects to the updated Table 5 for a comprehensive evaluation.

% We understand your concern about the impact of different target objects on our method. To illustrate the robustness of our algorithm, we performed experiments using diverse objects from the Stanford repository, namely the bunny and the dragon. The outcome of these experiments are presented in Table~\ref{tab:r2}, showing that the object has little influence on our results. We will revise Table 5 to include more real-world objects.

\noindent \textbf{Different settings impacts performance.}
In Table 1, the '-Real' model was trained and tested on TUD-L's real scene data, corresponds to the 'seen' object setting. On the other hand, the '-AutoSynth' model, trained on synthetic data and tested on TUD-L's real scene data, represents an 'unseen' object setting. This discrepancy in settings accounts for the observed performance difference. The same principle applies to Tables 2 and 3, which were tested using the LM and LMO datasets. We will clarify this to avoid any confusion.

% The model marked by '-Real' in Table 1 is trained and tested on the TUD-L provided real scene data, which 
% which corresponds to the \emph{'seen'} object setting.  
% Conversely, the model marked by '-AutoSynth' is trained on the searched synthetic data by our pipeline but tested on the TUD-L real scene dataset, which is tested in the \emph{'unseen'} object setting, i.e., observing new objects at test time. This fundamental difference in data settings is primarily responsible for the observed performance gap. We will clarify this in the final version.
% The model trained on the real data employs the same object for training and testing, 

\noindent \textbf{Evaluation of alternative surrogate networks.} 
Following the reviewer's suggestion, we experimented with the method from~[1], which introduces an auxiliary network intended to extract useful features for tasks such as shape classification and 3D keypoint prediction.
However, the high computational cost of this model was a concern. A full search would require around 34.65 GPU days on an Nvidia-V100 GPU, marking it 75 times slower than our approach. This evidences a key advantage of using a simple auto-encoder as surrogate model.
\input{table/rebuttal_R2}

% Thanks for your valuable suggestion. We believe that the using the SSL model~[1] indeed can mitigates the issue that less training data less generalization on test data, as SSL model can utilize beyond labeled training data. While it is a constructive idea, the main constraint is its high computational cost. A single trial requires about 250 mins and 9GB of GPU memory, equating to around 34.65 GPU days on a V100 for all 1,000 trials. This makes it around 75 times slower than our method. Despite this, we recognize its potential and intend to incorporate it in our final paper.



% We experimented with the method detailed in paper~\cite{Poursaeed20}, which introduced an auxiliary network intended to extract useful features for tasks like shape classification and 3D keypoint prediction. This suggests the auxiliary network could potentially pair well with these tasks and serve as an effective surrogate network.

% However, the primary concern was the computational cost, both in terms of time and memory. A single trial took approximately 250 minutes and utilized 9GB of GPU memory. Given these constraints, completing all trials in a single search process would equate to approximately 34.65 GPU days on an Nvidia-V100 GPU. This is significantly less efficient, being roughly 75 times slower than our proposed method.



% [1] Self-Supervised Learning of Point Clouds via Orientation Estimation

% [RED] Try the SSL 3D task. If the network is too large, then it's a very good excuse. We will include this result and further clarify this part in the final reviewed version.

% [Table] [Single]

% Surrogate result [already have]

% BPNet result [already have]

% SSL task result [already have] 250 min

==> rebuttal_tex_iccv/R3.tex <==

\noindent \textbf{To R3}

%\noindent \textbf{Evaluation on other networks.} We agree that demonstrating our method's impact on other learning-based methods would strengthen our claim. We plan to add more such examples in our revised experiments.

%\noindent \textbf{Domain gap agnostic baseline.} Indeed, testing our method on learning methods that are agnostic to the domain gap would further underline its effectiveness. The domain gap remains a significant challenge for existing object-level registration methods. In paper, we utilized BPNet[1] as main baseline, given its effectiveness. If there are potential alternatives, we'd be open to conducting further experiments.

\noindent \textbf{Evaluation on other networks. Domain gap agnostic baseline.}
Indeed, exploring our method's effect on other learning approaches would add weight to our results. We selected BPNet as our baseline due to its performance on real scene data and robustness to domain gaps. We acknowledge that many methods, including FMR as indicated in Table~\ref{tab:r1}, have potential but may require modifications for handling real scene data effectively. We would nonetheless gladly experiment with alternative methods should the reviewer have specific suggestions.

% We used BPNet as baseline in our paper because of its effectiveness on real scene data and its robustness to domain gaps. We agree that demonstrating our method's impact on other learning-based methods would strengthen our claim. However, most methods struggle to handle the real scene data, and thus, although an improvement can be achieved, as shown for FMR in Table~\ref{tab:r1}, the accuracy remains altogether low. We would nonetheless gladly experiment with alternative methods should the reviewer have specific suggestions.

\noindent \textbf{Tackling other point cloud tasks.} 
Given that various tasks show similar responses to changing input data, we expect that our method could benefit other learning-based point cloud-related tasks facing a domain gap. Your suggestion presents an intriguing direction for future work.

% Given that various tasks show similar responses to changing input data, we expect that our method could benefit other learning-based point cloud-related tasks facing a domain gap. This goes beyond our focus but is an interesting future work direction.

\noindent \textbf{Bi-level searching policy.} Thank you for this insightful idea of tailoring policies for different testing datasets or different optimization stages. We agree that adapting the training dataset to the training process could potentially improve performance. How to do so remains an open question. We will explore this further and consider it for our future work.

\noindent \textbf{Discretizing the searching space.} The discretization size of the search space indeed impacts the performance. In Table~\ref{tab:r2} (AS-Shrink), we show that the performance drops as the search space shrinks. Here, we reduced the operation's interval from 9 to 4 results in $4^{11}=4194304$ possibilities. A fine-grained discretization yields more accurate results, but at the expense of computational efficiency. We will discuss this trade-off more explicitly in the final version.

{
\scriptsize
% \noindent [1] X. Huang et al. A comprehensive survey on point cloud registration. arXiv 2021
\noindent [1] O. Poursaeed et al.Self-supervised learning of point clouds via orientation estimation. 3D Vision 2020.
}

==> table/rebuttal_R1.tex <==
\vspace{-.7em}
\begin{table}[ht]
    \centering
    {\small
    
    \setlength{\tabcolsep}{2.2mm}{
    \begin{tabular}{l|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c}{Translation mAP} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$\\
        \midrule
        FMR(MN40)    & 0.02 & 0.03 & 0.04 & 0.03 & 0.12 & 0.67 \\
        FMR(search) & 0.03 & 0.05 & 0.07 & 0.03 & 0.18 & 0.75 \\
        \bottomrule
    \end{tabular}
    }}
    \vspace{2pt}
    \caption{FMR trained on different datasets and tested on TUD-L.}
    \label{tab:r1}
\end{table}
\vspace{-0.8em}

==> table/rebuttal_R2.tex <==
\vspace{-.9em}
\begin{table}[ht]
    \centering
    {\small
    \setlength{\tabcolsep}{2.2mm}{
    \begin{tabular}{l|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c}{Translation mAP} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$\\
        \midrule
        AS-Bunny    & 0.78 & 0.81 & 0.85 & 0.77 & 0.86 & 0.95 \\
        AS-Dragon   & 0.77 & 0.80 & 0.82 & 0.77 & 0.85 & 0.94 \\
        \midrule
        AS-Angle    & 0.61 & 0.64 & 0.66 & 0.62 & 0.73 & 0.87 \\
        AS-Shrink   & 0.64 & 0.67 & 0.69 & 0.64 & 0.75 & 0.92 \\
        \bottomrule
    \end{tabular}
    }}
    \vspace{3pt}
    \caption{Evaluation with different target datasets and settings.}
    \label{tab:r2}
\end{table}
\vspace{-1.em}

==> table/syn_datasets.tex <==
\begin{table}[!ht]
    \centering
    {% \scriptsize
    \setlength{\tabcolsep}{1.mm}{
    \begin{tabular}{l|ccc|ccc|c}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{1}{c}{ADD} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & $0.1d$ \\
        \midrule
        ShapeNetCoreV2      & 0.67 & 0.70 & 0.73 & 0.67 & 0.77 & 0.87 & 0.73 \\
        ModelNet40          & 0.71 & 0.74 & 0.77 & 0.70 & 0.80 & 0.94 & 0.76 \\
        AutoSynth           & 0.78 & 0.81 & 0.85 & 0.77 & 0.86 & 0.95 & 0.84 \\
        \bottomrule
    \end{tabular}
    }}
    \caption{Comparison of BPNet trained with different synthetic datasets and evaluated on the TUD-L dataset.}
    \label{tab:syn_datasets}
\end{table}

==> table/target_dataset.tex <==
\begin{table}[!t]
    \centering
    {% \scriptsize
    \setlength{\tabcolsep}{1.mm}{
    \begin{tabular}{l|ccc|ccc|c}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{1}{c}{ADD} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & $0.1d$ \\
        \midrule
        MN40-one     & 0.76 & 0.80 & 0.84 & 0.77 & 0.86 & 0.93 & 0.82 \\ % iter_50000.pth.tar
        % MN40-one-original   & 0.59 & 0.62 & 0.68 & 0.59 & 0.71 & 0.92 & 0.65 \\
        MN40-full      & 0.76 & 0.80 & 0.83 & 0.76 & 0.86 & 0.96 & 0.83 \\ % iter_29000.pth.tar
        % MN40-full-original    & 0.71 & 0.74 & 0.77 & 0.70 & 0.80 & 0.94 & 0.76 \\
        Stanford-Bunny          & \textbf{0.78} & \textbf{0.81} & \textbf{0.85} & \textbf{0.77} & \textbf{0.86} & \textbf{0.95} & \textbf{0.84} \\
        \bottomrule
    \end{tabular}
    }}
    \caption{Impact of the target dataset. While using the real-scan Stanford Bunny as target data during the search yields the best results, our method is robust to the use of different target datasets.}
    \label{tab:target_dataset}
\end{table}

==> table/tendency_full.tex <==
\begin{table*}[!t]
    \centering
    {%\scriptsize
    \setlength{\tabcolsep}{2.67mm}{
    \begin{tabular}{l|c|ccc|ccc|c|cccc}
        \toprule
        & \multicolumn{1}{c|}{Method} & \multicolumn{7}{c|}{BPNet} & \multicolumn{1}{c}{AutoEncoder} \\
        \midrule
        \multicolumn{1}{c|}{} & & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{1}{c|}{ADD} & \multicolumn{1}{c}{Recontruction} \\
        \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{c|}{Setting}  & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & $0.1d$ & Chamfer Dist\\
        \midrule
        \multirow{6}{*}{TUD-L} 
        & MN40(01\_per\_cate)         & 0.59 & 0.62 & 0.68 & 0.59 & 0.71 & 0.92 & 0.65 & 22.27 \\ % ckpt/SA_modelnet_01_per_category/ckpt_best.pth.tar
        & MN40(05\_per\_cate)         & 0.61 & 0.66 & 0.69 & 0.62 & 0.74 & 0.90 & 0.68 & 17.81 \\ 
        & MN40(10\_per\_cate)         & 0.66 & 0.70 & 0.73 & 0.66 & 0.82 & 0.92 & 0.72 & 9.97 \\ % ckpt/SA_modelnet_10_per_category_random/iter_41000.pth.tar
        & MN40(50\_per\_cate)         & 0.69 & 0.72 & 0.75 & 0.69 & 0.81 & 0.91 & 0.75 & 6.82 \\  % Latest
        & MN40-full                   & 0.71 & 0.74 & 0.77 & 0.70 & 0.80 & 0.94 & 0.76 & 6.65 \\
        & AutoSynth                      & 0.78 & 0.81 & 0.85 & 0.77 & 0.86 & 0.95 & 0.84 & 4.16  \\
        \midrule
        \multirow{6}{*}{LM} 
        & MN40(01\_per\_cate)        & 0.25 & 0.35 & 0.44 & 0.33 & 0.66 & 0.92 & 0.37 & 33.28 \\
        & MN40(05\_per\_cate)        & 0.27 & 0.38 & 0.46 & 0.35 & 0.68 & 0.94 & 0.39 & 26.01 \\
        & MN40(10\_per\_cate)        & 0.29 & 0.41 & 0.49 & 0.37 & 0.71 & 0.95 & 0.42 & 12.12 \\ 
        & MN40(50\_per\_cate)        & 0.31 & 0.43 & 0.52 & 0.37 & 0.69 & 0.94 & 0.44 & 9.83 \\ %latest
        & MN40-full                  & 0.31 & 0.42 & 0.50 & 0.37 & 0.69 & 0.95 & 0.43 & 9.59 \\
        & AutoSynth                     & 0.36 & 0.49 & 0.58 & 0.40 & 0.74 & 0.93 & 0.50 & 7.01 \\
        \midrule
        \multirow{6}{*}{LMO} 
        & MN40(01\_per\_cate)          & 0.12 & 0.19 & 0.23 & 0.21 & 0.57 & 0.87 & 0.21 & 31.54 \\
        & MN40(05\_per\_cate)          & 0.16 & 0.26 & 0.35 & 0.26 & 0.61 & 0.90 & 0.28 & 23.47 \\
        & MN40(10\_per\_cate)          & 0.20 & 0.29 & 0.36 & 0.29 & 0.60 & 0.91 & 0.29 & 11.58 \\
        & MN40(50\_per\_cate)          & 0.22 & 0.33 & 0.43 & 0.27 & 0.61 & 0.92 & 0.34 & 9.45 \\
        & MN40-full                    & 0.22 & 0.32 & 0.41 & 0.30 & 0.63 & 0.92 & 0.34 & 9.42 \\
        & AutoSynth                       & 0.25 & 0.35 & 0.41 & 0.34 & 0.65 & 0.92 & 0.37 & 6.43 \\
        \bottomrule
    \end{tabular}
    }}
    \caption{
    Quantitative comparison of BPNet trained with different dataset settings and evaluated on the \textbf{TUD-L, LINEMOD, and Occluded-LINEMOD} real scene datasets. For the ModelNet40, we pick 1, 5, 10 and 50 mesh models from each category, corresponding to 40, 200, 400, 2000 mesh models.
    The Chamfer distance is multiplied by $10^3$. Note that, for both registration and reconstruction, increasing the number of training mesh models improves the performance. 
    %\MS{If we need to save space, we could keep only one dataset here and move the other two to the supplementary materia.}
    }
    \label{tab:tendency_full}
    % \vspace{-2.25em}
\end{table*}
